Electron transfer efficiency in liquid xenon across THGEM holes

Dual-phase liquid-xenon time projection chambers (LXe TPCs) deploying a few tonnes of liquid are presently leading the search for WIMP dark matter. Scaling these detectors to 10-fold larger fiducial masses, while improving their sensitivity to low-mass WIMPs presents difficult challenges in detector design. Several groups are considering a departure from current schemes, towards either single-phase liquid-only TPCs, or dual-phase detectors where the electroluminescence region consists of patterned electrodes. Here, we discuss the possible use of Thick Gaseous Electron Multipliers (THGEMs) coated with a VUV photocathode and immersed in LXe as a building block in such designs. We focus on the transfer efficiencies of ionization electrons and photoelectrons emitted from the photocathode through the electrode holes, and show experimentally that efficiencies approaching 100 % can be achieved with realistic voltage settings. The observed voltage dependence of the transfer efficiencies is consistent with electron transport simulations once diffusion and charging-up effects are included.

==> src/leftovers.tex <==

\subsection*{Setup for the photoemission measurement.}
{\color{red} Probably not relevant? Discard? We also have a measurement of photoemission with the S1 setup}

This setup, depicted in Figure \ref{fig:photoemission_setup}, consisted of a 20-mm diameter quartz window mounted on a stainless steel plate.
The window was coated first with a layer of $\sim$20 nm of Cr to obtain a conductive surface.
The edges of the window were coated with conductive epoxy to bridge the gap to the frame and ensure a good electrical contact.
On top of the metal coating, we deposited a 50-nm-thick layer of CsI by evaporation.
3 mm above this frame, we placed the THGEM without any coating.
On top of the THGEM, also at a 3 mm distance, we placed a mesh.
The setup is illuminated externally by a H$_2$ lamp through the viewport using an optical fiber.

\begin{figure}
    \centering
    \includegraphics[height=6cm]{img/photoemission_setup.png}
    \caption{Schematic diagram of the setup used for the photoemission measurement.}
    \label{fig:photoemission_setup}
\end{figure}



\ignoreblock
{
\subsection*{Setup for the extraction measurement}

The measurement of the electron extraction into gas phase consists of an alpha source held in a metallic frame and a mesh that are fully immerse in liquid.
In the gas phase we place a THGEM and the interface lies somewhere in between the mesh and the THGEM.
This scheme is depicted in Figure \ref{fig:extraction_setup}.
The mesh above the source that the field across the interface is homogeneous.
Finally, by using a THGEM we are able to apply a reverse field between both sides of the electrode, ensuring that the electrons are not dispersed sideways, as they are focused into the bottom plane.

\begin{figure}
    \centering
    \includegraphics[height=6cm]{img/extraction_setup.png}
    \caption{Schematic diagram of the setup used for the extraction efficiency measurement.}
    \label{fig:extraction_setup}
\end{figure}
}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{img/photoemission.png}
    \caption{{\color{red}
    This is one of our photoemission measurements, but does it fit in this paper? probably not}
}
    \label{fig:photoemission}
\end{figure}

